APAR: Modeling Irregular Target Functions in Tabular Regression via Arithmetic-Aware Pre-Training and Adaptive-Regularized Fine-Tuning

Tabular data are fundamental in common machine learning applications, ranging from finance to genomics and healthcare. This paper focuses on tabular regression tasks, a field where deep learning (DL) methods are not consistently superior to machine learning (ML) models due to the challenges posed by irregular target functions inherent in tabular data, causing sensitive label changes with minor variations from features. To address these issues, we propose a novel Arithmetic-Aware Pre-training and Adaptive-Regularized Fine-tuning framework (APAR), which enables the model to fit irregular target function in tabular data while reducing the negative impact of overfitting. In the pre-training phase, APAR introduces an arithmetic-aware pretext objective to capture intricate sample-wise relationships from the perspective of continuous labels. In the fine-tuning phase, a consistency-based adaptive regularization technique is proposed to self-learn appropriate data augmentation. Extensive experiments across 10 datasets demonstrated that APAR outperforms existing GBDT-, supervised NN-, and pretrain-finetune NN-based methods in RMSE (+9.43% $\sim$ 20.37%), and empirically validated the effects of pre-training tasks, including the study of arithmetic operations. Our code and data are publicly available at https://github.com/johnnyhwu/APAR.

==> src/solution/impl_detail.tex <==
\subsection{Implementation Details}
\label{sec:aridaformer_impl}
We implemented our proposed AridaFormer approach using PyTorch version 1.13.1 and conducted training on a 64-bit Linux server featuring 48 Intel Xeon CPUs running at 2.10GHz, 256GB of memory, and a single NVIDIA GeForce RTX 3090 GPU.

==> src/solution/summary.tex <==
\subsection{Discussion}
APAR is based on a Transformer architecture adapted to tabular data to address challenges such as feature heterogeneity, uninformativeness, and rotational invariance. Our primary focus, however, is on navigating irregular target functions. The often non-smooth mapping between features and targets can lead to overfitting, as models may rely too heavily on individual samples or features. Our approach addresses this issue through two key strategies:
Firstly, during the pre-training phase, we introduce an arithmetic-aware task that constructs arithmetic tasks using regression labels. This encourages the model to consider a broader range of samples, fostering a more generalized understanding of the dataset. This strategy emphasizes the importance of capturing relationships among samples to learn better representation of individual samples by leveraging regression labels, an aspect often overlooked in previous methods.
Secondly, in the fine-tuning phase, we implement consistency-based adaptive regularization. This method penalizes inconsistencies in predictions across original sample and augmented sample, enabling the model to autonomously learn effective data augmentation. This reduces the likelihood of human-designed augmentations inadvertently degrading model performance, making the difference from traditional methods.
In summary, our combination of arithmetic-aware pre-training and adaptive regularization provides a comprehensive framework that effectively addresses the challenges associated with irregular target functions, enhancing existing methodologies in the field.

% The challenge with irregular target functions is their non-smooth mapping between features and targets, leading to the risk of overfitting, as models may focus too narrowly on individual samples or features to capture complex patterns.
% During the pre-training phase, our arithmetic-aware task utilizes regression labels to construct arithmetic tasks, encouraging the model to consider a broader set of samples rather than isolated ones. This approach fosters a more generalized understanding of the data.
% Furthermore, in the fine-tuning phase, our adaptive consistency-based regularization targets the model's reliance on individual features. It penalizes inconsistencies in predictions across augmented samples, and allows the model to learn effective data augmentation strategies autonomously. This reduces the likelihood of human-designed augmentations inadvertently degrading model performance.
% Both arithmetic-aware pre-training (AP) and adaptive regularization (AR) encourage the integration of multiple samples and features into the model's analysis, mitigating the risk of overfitting to complex patterns inherent in irregular target functions. 


